Optimal Power Flow with Inelastic Demands for Demand Response in Radial Distribution Networks

The classical optimal power flow problem optimizes the power flow in a power network considering the associated flow and operating constraints. In this paper, we investigate optimal power flow in the context of utility-maximizing demand response management in distribution networks, in which customers' demands are satisfied subject to the operating constraints of voltage and transmission power capacity. The prior results concern only elastic demands that can be partially satisfied, whereas power demands in practice can be inelastic with binary control decisions, which gives rise to a mixed integer programming problem. We shed light on the hardness and approximability by polynomial-time algorithms for optimal power flow problem with inelastic demands. We show that this problem is inapproximable for general power network topology with upper and lower bounds of nodal voltage. Then, we propose an efficient algorithm for a relaxed problem in radial networks with bounded transmission power loss and upper bound of nodal voltage. We derive an approximation ratio between the proposed algorithm and the exact optimal solution. Simulations show that the proposed algorithm can produce close-to-optimal solutions in practice.

==> bio.tex <==
%\vspace{200pt}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/majid.png}}]%
	{Majid Khonji} received the B.S. degree in software engineering from UAE University, UAE, in 2007 and the M.S. degree in Security, Cryptology and Coding of Information Systems from Ensimag, Grenoble Institute of Technology, France, and the Ph.D. degree in interdisciplinary engineering from Masdar Institute of Science and Technology in 2016. He is currently a Senior R\&D Researcher in Dubai Electricity and Water Authority (DEWA). His research interests are in algorithms, optimization, artificial intelligence, and smart grid.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/ckchau.jpg}}]{Chi-Kin Chau}
is an assistant professor at the Dept. of EECS of Masdar Institute of Science and Technology in Abu Dhabi, UAE. He researches in broad areas of intelligent systems, optimization and algorithms for applications of sustainability and energy systems (e.g., smart buildings, smart grid and intelligent vehicles). Previously, He was a visiting professor at MIT, and a senior research fellow at the Institute for Infocomm Research (I$^2$R) of A*STAR in Singapore. He was awarded a Croucher Foundation Research Fellowship at the EE Dept., University College London. He was a visiting scholar at IBM T. J. Watson Research Center (Hawthorne, US), and Raytheon-BBN Technologies (Boston, US). He received the Ph.D. from University of Cambridge and B.Eng. from the Chinese University of Hong Kong. He has been a TPC member for a number of international conferences in energy systems, such as ACM e­Energy and IEEE SmartGridComm. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig/image001.png}}]%
	{Khaled Elbassioni} is an associate professor at Masdar Institute. He received B.S. and M.S. degrees in Computer Science from Alexandria University, Egypt, and a Ph.D. degree in Computer Science from Rutgers University, USA.  From 2006 to 2012, he was a senior researcher at Max-Planck Institute for Informatics, Saarbruecken, Germany.
\end{IEEEbiography}

\vfill
